Control-oriented Clustering of Visual Latent Representation

We initiate a study of the geometry of the visual representation space -- the information channel from the vision encoder to the action decoder -- in an image-based control pipeline learned from behavior cloning. Inspired by the phenomenon of neural collapse (NC) in image classification (arXiv:2008.08186), we empirically demonstrate the prevalent emergence of a similar law of clustering in the visual representation space. Specifically, in discrete image-based control (e.g., Lunar Lander), the visual representations cluster according to the natural discrete action labels; in continuous image-based control (e.g., Planar Pushing and Block Stacking), the clustering emerges according to "control-oriented" classes that are based on (a) the relative pose between the object and the target in the input or (b) the relative pose of the object induced by expert actions in the output. Each of the classes corresponds to one relative pose orthant (REPO). Beyond empirical observation, we show such a law of clustering can be leveraged as an algorithmic tool to improve test-time performance when training a policy with limited expert demonstrations. Particularly, we pretrain the vision encoder using NC as a regularization to encourage control-oriented clustering of the visual features. Surprisingly, such an NC-pretrained vision encoder, when finetuned end-to-end with the action decoder, boosts the test-time performance by 10% to 35%. Real-world vision-based planar pushing experiments confirmed the surprising advantage of control-oriented visual representation pretraining.

==> sections/app-block_stacking.tex <==
%!TEX root = ../main.tex

\rv{
\section{Block Stacking Experiment Details}
\label{app:app_block_stacking}


\paragraph{Setup} Designed by~\citet{mandlekar2023mimicgen}, the block stacking is implemented as one of the manipulation tasks in MimicGen dataset using robosuite framework~\citep{zhu2020robosuite}
backended on MuJoCo~\citep{todorov2012mujoco}. The goal of the task is to grasp and place the red cube on the green cube given randomly initialized positions of two cubes on a table. To train the imitation learning pipeline, we used the dataset ``core stack_d0'' provided by MimicGen which contains 1000 demos as our expert training dataset.

\paragraph{Labeling Details} Similar to the goal-based and action-based methods designed in planar pushing task, we still computed and assigned a label for each training sample based on the triplet $(x, y, \theta)$. The only difference for action-based metric is that the object of relative pose has changed from the pushed block to the grasped red cube. This also applies to the object for goal-based metric and besides the target has updated to the bottom green cube.

\paragraph{Training Details} We used ResNet18 as the vision encoder and diffusion model as the action decoder. The action space is characterized by a 7-dimensional continuous vector, corresponding to the seven degrees of freedom (DoF) of the simulated Franka Emika robot arm used in the block stacking task. To keep the consistency with the planar pushing task, we applied the same observation and prediction horizon along with the same training hyperparameters as mentioned in Appendix~\ref{app:app_planar_pushing}. 
}


==> sections/app-double-integrator.tex <==
%!TEX root = ../main.tex

\section{Experimental details: minimum-time double integrator}
\label{app:double-integrator}

\begin{itemize}
    \item What is the value of $N$?
    \hq{N=5000.}
    
    \item How did you sample $x$? I think a good strategy is to uniformly sample inside a ball centered at $0$ with radius $10$. 
    \hq{The points are sampled inside a ball centered at $0$ with radius $10$. Then N more (0,0) points are added extraly.}

    \item Can you plot the \emph{training loss} and \emph{classification error}, both with respect to training epoches? Training loss means the cross-entropy loss, and classification error means error rate of classification (for example ``predicting $0$ or $+1$ but the true label is $-1$'' is a wrong classification; among the $3N$ training samples, if $N$ predicted labels are wrong, then the classification error rate is $\frac{1}{3} = \frac{N}{3N}$). 
    \hq{Included in the result folder.}
\end{itemize}

==> sections/app-neural-collapse-metric.tex <==
%!TEX root = ../main.tex

\section{Neural Collapse Metric}

$N_c$: number of samples in class $c$ with $c\in [C]$. Class mean vector: 
$$
\mu^{c} = \frac{1}{N_c}\sum_{i=1}^{N_c} f_{i}^{c}, c= 1,\dots,C.
$$
Let $N := N_1 + \dots + N_C$ be the total number of samples, the global mean vector is
$$
\mu = \frac{1}{N}\sum_{c=1}^C\sum_{i=1}^{N_c} f_{i}^{c}.
$$
Let $\tilde{\mu}^c := \mu^c - \mu$ be the globally-centered class means, and $\tilde{f}^c_i:=f^c_i - \mu$ be the globally-centered feature vectors. We evaluate neural collapse using the following two metrics.
\begin{enumerate}
    \item NC1: Within-class variability collapse. Referenced from 3.4 Signal-to-Noise Ratio of paper \cite{wu2024linguistic}. 
    We use the class-distance normalized variance (CDNV) to measure within-class variability collapse(NC1), depending on the ratio of within-class to between-class variabilities \cite{wu2024linguistic}. 
    $$
    \sigma_c^2:=\frac{1}{N_c-1} \sum_{i=1}^{N_c} \|\tilde{f}^c_i-\tilde{\mu}^c\|_2^2 
    $$
    $$
    \operatorname{CDNV}_{c,c^{\prime}}:=
    \frac{\sigma_c^2+\sigma_{c^{\prime}}^2}{2\left\|\tilde{\mu}^c-\tilde{\mu}^{c^{\prime}}\right\|_2^2}, \quad \forall c \neq c^{\prime}
    $$

     Within-class variability collapse is then re-characterized by the minimization of this quantity: $ \text{CDNV}_{c,c'} \rightarrow 0, \forall  c \neq c' $. 
     
     % \hy{what is CDNV short for?} \hq{Just added the full definition for CDNV here.}

    \item NC2: Convergence to Simplex ETF. Reference from paper \cite{papyan2020prevalence}.
     % \hy{You have a vector divided by a vector, what does that mean?} \hq{Sorry it's a typo, I meant by the length of the vectors. And here is an explanation about why I used division instead of the original definition in referenced paper: The original paper uses this definition to compare lengths of globally centered mean vectors: $|\|\tilde{\mu}^c\|_2 - \|\tilde{\mu}^{c^{\prime}}\|_2|$. But I think the drawback of this is that for a bad feature embedding space, it usually has smaller scale compared to a good feature embedding space. This means that the differences for bad feature embedding space would naturally be smaller than a good one. So I think it is not a fair comparison. If we change it to ratio, it would avoid this problem. And in this case, the length of globally centered mean vector would never be zero. So it would not cause any error by using division.   }
    $$
    \text{NC2-Norm-Deviation} = 
    \frac{\text{std}\{\|\tilde{\mu}^c\|_2\}}{\text{mean}\{\|\tilde{\mu}^c\|_2\}},  c\in [C]
    $$
    One aspect of convergence to simplex ETF is measured by minimizing NC2-Norm-Deviation.
    
    
    
    $$
    \bar{\mu}^c = \frac{\tilde{{\mu}}^c}{ \| \tilde{\mu}^c \|_2 } 
    $$
    

    $$
    \text{NC2-Angle-Deviation} = 
    \text{std}\{\langle \bar{\mu}^c, \bar{\mu}^{c'} \rangle \},  \forall c \neq c^{\prime} 
    $$

    Another aspect of convergence to simplex ETF is measured by minimizing NC2-Angle-Deviation.
    
    % \hy{general comment: do NOT rush through the math, expain everything you wrote, double check everything you wrote, ask chatGPT how to write math equations in Latex that look nice, be responsible for everything you wrote. A paper full of grammar and typesetting errors shows the authors are lazy and will drive the reviewers mad.}



\end{enumerate}

==> sections/app-planar_pushing.tex <==
%!TEX root = ../main.tex


\section{Planar Pushing Experiment Details}
\label{app:app_planar_pushing}

\paragraph{Setup} Please refer to \S\ref{sec:nc-observation-planar-pushing} in main paper.

\rv{
\paragraph{Labeling Details} In the planar pushing task, we designed two different 8-class labeling metrics (named \emph{goal-based} and \emph{action-based} metrics) to assign each training sample a unique class. The details of goal-based classification method could refer to \S\ref{sec:classification} and action-based could refer to Appendix~\ref{app:action_based_classfication}. In both methods, we computed a relative pose as triplet $(x, y, \theta)$ for each training sample and then we assigned the sample a corresponding label range from 0 to 7 based on the signs of each dimension.  
}

\paragraph{Training Details} We used ResNet18/DINOv2 as the vision encoder and diffusion model~(DM)/LSTM as the action decoder. This action dimension is 2 for planar pushing, representing the action (x,y) for the pusher(agent pose). With an observation horizon=2, each input image is encoded into 512 dimensional visual feature. We use long-horizon planning with prediction horizon=16. For training, with batch size of 64 we use the AdamW optimizer with learning rate 1e-4 and weight decay value 1e-6, and Cosine LR scheduler with linear warmup. This is consistent with the diffusion policy paper \cite{chi2023diffusion} and please refer to this paper if more additional model structure details are needed. 



==> sections/fig-nc-cross_domain_from_domain0_to_domain7.tex <==


\begin{figure}[h]
    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cccc}
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain0_to_domain7/test_score/from_domain0_to_domain_7_test_together_score.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain0_to_domain7/NC_input_space/from_domain0_to_domain_7_test_together_nc1_input_space.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain0_to_domain7/NC_input_space/from_domain0_to_domain_7_test_together_nc2angle_input_space.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain0_to_domain7/NC_input_space/from_domain0_to_domain_7_test_together_nc2norm_input_space.pdf}
            \end{minipage}
            \\
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain0_to_domain7/test_score/from_domain0_to_domain_7_test_together_score.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain0_to_domain7/NC_action_intention/from_domain0_to_domain_7_test_together_nc1_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain0_to_domain7/NC_action_intention/from_domain0_to_domain_7_test_together_nc2angle_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain0_to_domain7/NC_action_intention/from_domain0_to_domain_7_test_together_nc2angle_action_intention.pdf}
            \end{minipage}
        \end{tabular}
    \end{minipage}
    \caption{Neural collapse in planar pushing. (From domain 0 finetune to domain 7)
    \label{fig:nc-push_finetune_domain0_to_domain7}}
\end{figure}

==> sections/fig-nc-cross_domain_from_domain13_to_domain15.tex <==


\begin{figure}[h]
    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cccc}
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain13_to_domain15/test_score/from_domain13_to_domain_15_test_together_score.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain13_to_domain15/NC_input_space/from_domain13_to_domain_15_test_together_nc1_input_space.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain13_to_domain15/NC_input_space/from_domain13_to_domain_15_test_together_nc2angle_input_space.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain13_to_domain15/NC_input_space/from_domain13_to_domain_15_test_together_nc2norm_input_space.pdf}
            \end{minipage}
            \\
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain13_to_domain15/test_score/from_domain13_to_domain_15_test_together_score.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain13_to_domain15/NC_action_intention/from_domain13_to_domain_15_test_together_nc1_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain13_to_domain15/NC_action_intention/from_domain13_to_domain_15_test_together_nc2angle_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain13_to_domain15/NC_action_intention/from_domain13_to_domain_15_test_together_nc2angle_action_intention.pdf}
            \end{minipage}
        \end{tabular}
    \end{minipage}
    \caption{Neural collapse in planar pushing. (From domain 13 finetune to domain 15)
    \label{fig:nc-push_finetune_domain13_to_domain15}}
\end{figure}

==> sections/fig-nc-cross_domain_from_domain18_to_domain0.tex <==


\begin{figure}[h]
    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cccc}
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain18_to_domain0/test_score/from_domain18_to_domain_0_test_together_score.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain18_to_domain0/NC_input_space/from_domain18_to_domain_0_test_together_nc1_input_space.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain18_to_domain0/NC_input_space/from_domain18_to_domain_0_test_together_nc2angle_input_space.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain18_to_domain0/NC_input_space/from_domain18_to_domain_0_test_together_nc2norm_input_space.pdf}
            \end{minipage}
            \\
            
        \end{tabular}
    \end{minipage}
    \caption{Neural re-collapse in planar pushing. (From domain 18 finetune to domain 0)
    \label{fig:nc-cross-domains}}
\end{figure}

==> sections/fig-nc-cross_domain_from_domain7_to_domain13.tex <==


\begin{figure}[h]
    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cccc}
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain7_to_domain13/test_score/from_domain7_to_domain_13_test_together_score.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain7_to_domain13/NC_input_space/from_domain7_to_domain_13_test_together_nc1_input_space.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain7_to_domain13/NC_input_space/from_domain7_to_domain_13_test_together_nc2angle_input_space.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain7_to_domain13/NC_input_space/from_domain7_to_domain_13_test_together_nc2norm_input_space.pdf}
            \end{minipage}
            \\
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain7_to_domain13/test_score/from_domain7_to_domain_13_test_together_score.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain7_to_domain13/NC_action_intention/from_domain7_to_domain_13_test_together_nc1_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain7_to_domain13/NC_action_intention/from_domain7_to_domain_13_test_together_nc2angle_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/continously_finetune/from_domain7_to_domain13/NC_action_intention/from_domain7_to_domain_13_test_together_nc2angle_action_intention.pdf}
            \end{minipage}
        \end{tabular}
    \end{minipage}
    \caption{Neural collapse in planar pushing. (From domain 7 finetune to domain 13)
    \label{fig:nc-push_finetune_domain7_to_domain13}}
\end{figure}

==> sections/fig-nc-push-input_500demos_dinov2_diffusion.tex <==


\begin{figure}[H]
    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cccc}
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/score/upload_domain18_dinov2_diffusion_result_preview_seed1-3.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_input_space_fixed_range/upload_domain18_dinov2_diffusion_result_preview_nc1_input_space_fixed_range.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_input_space_fixed_range/upload_domain18_dinov2_diffusion_result_preview_nc2angle_input_space_fixed_range.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_input_space_fixed_range/upload_domain18_dinov2_diffusion_result_preview_nc2norm_input_space_fixed_range.pdf}
            \end{minipage}
            \\
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/score/upload_domain18_dinov2_diffusion_result_preview_seed1-3.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_action_intention/upload_domain18_dinov2_diffusion_result_preview_nc1_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_action_intention/upload_domain18_dinov2_diffusion_result_preview_nc2angle_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_action_intention/upload_domain18_dinov2_diffusion_result_preview_nc2norm_action_intention.pdf}
            \end{minipage}
        \end{tabular}
    \end{minipage}
    \caption{Neural collapse in planar pushing. (dinov2+diffusion)
    \label{fig:nc-push_500demos_dinov2_diffusion}}
\end{figure}

==> sections/fig-nc-push-input_500demos_dinov2_lstm.tex <==


\begin{figure}[H]
    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cccc}
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_lstm/score/upload_domain18_dinov2_lstm_result_preview_seed.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_lstm/NC_metric_input_space_fixed_range/upload_domain18_dinov2_lstm_result_preview_nc1_input_space_fixed_range.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_lstm/NC_metric_input_space_fixed_range/upload_domain18_dinov2_lstm_result_preview_nc2angle_input_space_fixed_range.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_lstm/NC_metric_input_space_fixed_range/upload_domain18_dinov2_lstm_result_preview_nc2norm_input_space_fixed_range.pdf}
            \end{minipage}
            \\
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_lstm/score/upload_domain18_dinov2_lstm_result_preview_seed.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_lstm/NC_metric_action_intention/upload_domain18_dinov2_lstm_result_preview_nc1_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_lstm/NC_metric_action_intention/upload_domain18_dinov2_lstm_result_preview_nc2angle_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_lstm/NC_metric_action_intention/upload_domain18_dinov2_lstm_result_preview_nc2norm_action_intention.pdf}
            \end{minipage}
        \end{tabular}
    \end{minipage}
    \caption{Neural collapse in planar pushing. (dinov2+lstm)
    \label{fig:nc-push_500demos_dinov2_lstm}}
\end{figure}

==> sections/fig-nc-push-input_500demos_resnet_dinov2_diffusion.tex <==


\begin{figure}[t]
    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccc}
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_resnet_diffusion/NC_metric_input_space_fixed_range/upload_domain18_resnet_diffusion_result_preview_nc1_input_space_fixed_range.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_resnet_diffusion/NC_metric_input_space_fixed_range/upload_domain18_resnet_diffusion_result_preview_nc2angle_input_space_fixed_range.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_resnet_diffusion/NC_metric_input_space_fixed_range/upload_domain18_resnet_diffusion_result_preview_nc2norm_input_space_fixed_range.pdf}
            \end{minipage}
            \\
            \multicolumn{3}{c}{\small (a-1) ResNet + DM, goal-based classification}
            \\
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_resnet_diffusion/NC_metric_action_intention/upload_domain18_resnet_diffusion_result_preview_nc1_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_resnet_diffusion/NC_metric_action_intention/upload_domain18_resnet_diffusion_result_preview_nc2angle_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_resnet_diffusion/NC_metric_action_intention/upload_domain18_resnet_diffusion_result_preview_nc2norm_action_intention.pdf}
            \end{minipage}
            \\
            \multicolumn{3}{c}{\small (a-2) ResNet + DM, action-based classification}
            \\
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_input_space_fixed_range/upload_domain18_dinov2_diffusion_result_preview_nc1_input_space_fixed_range.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_input_space_fixed_range/upload_domain18_dinov2_diffusion_result_preview_nc2angle_input_space_fixed_range.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_input_space_fixed_range/upload_domain18_dinov2_diffusion_result_preview_nc2norm_input_space_fixed_range.pdf}
            \end{minipage}
            \\
            \multicolumn{3}{c}{\small (b-1) DINOv2 + DM, goal-based classification}
            \\
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_action_intention/upload_domain18_dinov2_diffusion_result_preview_nc1_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_action_intention/upload_domain18_dinov2_diffusion_result_preview_nc2angle_action_intention.pdf}
            \end{minipage}
            &
            \hspace{-4mm}
            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figures/part3-NC_curve_during_training/500demos_dinov2_diffusion/NC_metric_action_intention/upload_domain18_dinov2_diffusion_result_preview_nc2norm_action_intention.pdf}
            \end{minipage}
            \\
            \multicolumn{3}{c}{\small (b-2) DINOv2 + DM, action-based classification}
        \end{tabular}
    \end{minipage}
    \vspace{-4mm}
    \caption{Prevalent emergence of neural collapse in the visual representation space. (a) Three NC metrics w.r.t. training epochs using ResNet as the vision encoder and diffusion model (DM) as the action decoder. (b) Three NC metrics w.r.t. training epochs using DINOv2 as the vision encoder and DM as the action decoder. All the plots show the mean and standard deviation (in shaded band) over three random seeds. The test scores are shown in Fig.~\ref{fig:test-scores}(a)(b). Similar observations of NC hold when replacing DM with LSTM as the action decoder, shown in Appendix~\ref{app:experiments}.
    \label{fig:nc-push_500demos_resnet_dinov2_diffusion}}
    \vspace{-6mm}
\end{figure}
